A stabilized computational nonlocal poromechanics model for dynamic analysis of saturated porous media

In this article we formulate a stable computational nonlocal poromechanics model for dynamic analysis of saturated porous media. As a novelty, the stabilization formulation eliminates zero-energy modes associated with the original multiphase correspondence constitutive models in the coupled nonlocal poromechanics model. The two-phase stabilization scheme is formulated based on an energy method that incorporates inhomogeneous solid deformation and fluid flow. In this method, the nonlocal formulations of skeleton strain energy and fluid flow dissipation energy equate to their local formulations. The stable coupled nonlocal poromechanics model is solved for dynamic analysis by an implicit time integration scheme. As a new contribution, we validate the coupled stabilization formulation by comparing numerical results with analytical and finite element solutions for one-dimensional and two-dimensional dynamic problems in saturated porous media. Numerical examples of dynamic strain localization in saturated porous media are presented to demonstrate the efficacy of the stable coupled poromechanics framework for localized failure under dynamic loads.

==> pd-stabilization.tex <==

@book{bobaru2016handbook,
  title={Handbook of peridynamic modeling},
  author={Bobaru, Florin and Foster, John T and Geubelle, Philippe H and Silling, Stewart A},
  year={2016},
  publisher={CRC press}
}

@book{madenci2014peridynamic,
  title={Peridynamic Theory and Its Applications},
  author={Madenci, Erdogan and Oterkus, Erkan},
  year={2014},
  publisher={Springer}
}

@article{markert2010comparison,
  title={Comparison of monolithic and splitting solution schemes for dynamic porous media problems},
  author={Markert, B and Heider, Y and Ehlers, W},
  journal={International journal for numerical methods in engineering},
  volume={82},
  number={11},
  pages={1341--1383},
  year={2010},
  publisher={Wiley Online Library}
}

@article{newmark1959method,
  title={A method of computation for structural dynamics},
  author={Newmark, Nathan M},
  journal={Journal of the engineering mechanics division},
  volume={85},
  number={3},
  pages={67--94},
  year={1959},
  publisher={American Society of Civil Engineers}
}

@article{hashim2020implicit,
  title={An implicit non-ordinary state-based peridynamics with stabilised correspondence material model for finite deformation analysis},
  author={Hashim, Nur A and Coombs, WM and Augarde, CE and Hattori, G},
  journal={Computer Methods in Applied Mechanics and Engineering},
  volume={371},
  pages={113304},
  year={2020},
  publisher={Elsevier}
}

@article{ni2020hybrid,
  title={Hybrid FEM and peridynamic simulation of hydraulic fracture propagation in saturated porous media},
  author={Ni, Tao and Pesavento, Francesco and Zaccariotto, Mirco and Galvanetto, Ugo and Zhu, Qi-Zhi and Schrefler, Bernhard A},
  journal={Computer Methods in Applied Mechanics and Engineering},
  volume={366},
  pages={113101},
  year={2020},
  publisher={Elsevier}
}

@article{turner2013non,
  title={A non-local model for fluid-structure interaction with applications in hydraulic fracturing},
  author={Turner, Daniel Z},
  journal={International Journal for Computational Methods in Engineering Science and Mechanics},
  volume={14},
  number={5},
  pages={391--400},
  year={2013},
  publisher={Taylor \& Francis}
}

@inproceedings{gabriel2004open,
  title={Open MPI: Goals, concept, and design of a next generation MPI implementation},
  author={Gabriel, Edgar and Fagg, Graham E and Bosilca, George and Angskun, Thara and Dongarra, Jack J and Squyres, Jeffrey M and Sahay, Vishal and Kambadur, Prabhanjan and Barrett, Brian and Lumsdaine, Andrew and others},
  booktitle={European Parallel Virtual Machine/Message Passing Interface Users’ Group Meeting},
  pages={97--104},
  year={2004},
  organization={Springer}
}

@book{schofield1968critical,
  title={Critical state soil mechanics},
  author={Schofield, Andrew and Wroth, Peter},
  year={1968},
  publisher={McGraw-hill}
}

@book{wood1990soil,
  title={Soil behaviour and critical state soil mechanics},
  author={Wood, David Muir},
  year={1990},
  publisher={Cambridge university press}
}

@book{borja2013plasticity,
  title={Plasticity: modeling \& computation},
  author={Borja, Ronaldo I},
  year={2013},
  publisher={Springer Science \& Business Media}
}

@book{simo1998computational,
  title={Computational inelasticity},
  author={Simo, Juan C and Hughes, Thomas JR},
  volume={7},
  year={1998},
  publisher={Springer Science \& Business Media}
}

@article{song2020peridynamic,
  title={On the peridynamic effective force state and multiphase constitutive correspondence principle},
  author={Song, Xiaoyu and Silling, Stewart A},
  journal={Journal of the Mechanics and Physics of Solids},
  volume={145},
  pages={104161},
  year={2020},
  publisher={Elsevier}
}

@article{borja2013shear,
  title={Shear band in sand with spatially varying density},
  author={Borja, Ronaldo I and Song, Xiaoyu and Rechenmacher, Amy L and Abedi, Sara and Wu, Wei},
  journal={Journal of the Mechanics and Physics of Solids},
  volume={61},
  number={1},
  pages={219--234},
  year={2013},
  publisher={Elsevier}
}

@article{song2014mathematical,
  title={Mathematical framework for unsaturated flow in the finite deformation range},
  author={Song, Xiaoyu and Borja, Ronaldo I},
  journal={International Journal for Numerical Methods in Engineering},
  volume={97},
  number={9},
  pages={658--682},
  year={2014},
  publisher={Wiley Online Library}
}

@book{hughes2012finite,
  title={The finite element method: linear static and dynamic finite element analysis},
  author={Hughes, Thomas JR},
  year={2012},
  publisher={Courier Corporation}
}

@book{cheng2016poroelasticity,
  title={Poroelasticity},
  author={Cheng, Alexander H-D},
  volume={27},
  year={2016},
  publisher={Springer}
}

@book{hughes2012finite,
  title={The finite element method: linear static and dynamic finite element analysis},
  author={Hughes, Thomas JR},
  year={2012},
  publisher={Courier Corporation}
}

@book{cheng2016poroelasticity,
  title={Poroelasticity},
  author={Cheng, Alexander H-D},
  volume={27},
  year={2016},
  publisher={Springer}
}

@article{turner2013non,
  title={A non-local model for fluid-structure interaction with applications in hydraulic fracturing},
  author={Turner, Daniel Z},
  journal={International Journal for Computational Methods in Engineering Science and Mechanics},
  volume={14},
  number={5},
  pages={391--400},
  year={2013},
  publisher={Taylor \& Francis}
}

@article{menon2019coupled,
  title={Coupled Analysis of Desiccation Cracking in Unsaturated Soils through a Non-Local Mathematical Formulation},
  author={Menon, Shashank and Song, Xiaoyu},
  journal={Geosciences},
  volume={9},
  number={10},
  pages={428},
  year={2019},
  publisher={Multidisciplinary Digital Publishing Institute}
}

@article{song2020peridynamic,
  title={On the peridynamic effective force state and multiphase constitutive correspondence principle},
  author={Song, Xiaoyu and Silling, Stewart A},
  journal={Journal of the Mechanics and Physics of Solids},
  volume={145},
  pages={104161},
  year={2020},
  publisher={Elsevier}
}

@article{menon2020computational,
  title={A computational periporomechanics model for localized failure in unsaturated porous media},
  author={Menon, Shashank and Song, Xiaoyu},
  journal={arXiv preprint arXiv:2010.15793},
  year={2020}
}

@article{alonso2021triggering,
  title={Triggering and motion of landslides},
  author={Alonso, Eduardo E},
  journal={G{\'e}otechnique},
  volume={71},
  number={1},
  pages={3--59},
  year={2021},
  publisher={Thomas Telford Ltd}
}

@book{lewis1998finite,
  title={The finite element method in the static and dynamic deformation and consolidation of porous media},
  author={Lewis, Roland Wynne and Schrefler, Bernard A},
  number={BOOK},
  year={1998},
  publisher={John Wiley}
}

@article{RoyChowdhury2019modified,
author = {{Roy Chowdhury}, Shubhankar and Roy, Pranesh and Roy, Debasish and Reddy, J. N.},
journal = {Computer Methods in Applied Mechanics and Engineering},
pages = {530--549},
publisher = {Elsevier B.V.},
title = {{A modified peridynamics correspondence principle: Removal of zero-energy deformation and other implications}},
volume = {346},
year = {2019}
}

@article{Wu2015stabilized,
author = {Wu, C. T. and Ren, B.},
journal = {Computer Methods in Applied Mechanics and Engineering},
month = {jul},
pages = {197--215},
publisher = {Elsevier},
title = {{A stabilized non-ordinary state-based peridynamics for the nonlocal ductile material failure analysis in metal machining process}},
volume = {291},
year = {2015}
}

@article{Li2018stabilized,
author = {Li, P. and Hao, Z. M. and Zhen, W. Q.},
journal = {Computer Methods in Applied Mechanics and Engineering},
month = {sep},
pages = {262--280},
publisher = {Elsevier B.V.},
title = {{A stabilized non-ordinary state-based peridynamic model}},
volume = {339},
year = {2018}
}

@article{vardoulakis1986dynamic,
  title={Dynamic stability analysis of undrained simple shear on water-saturated granular soils},
  author={Vardoulakis, I},
  journal={International journal for numerical and analytical methods in geomechanics},
  volume={10},
  number={2},
  pages={177--190},
  year={1986},
  publisher={Wiley Online Library}
}

@article{Loret1991Dynamic,
  title={Dynamic strain localization in fluid-saturated porous media},
  author={Loret, B and Prevost, Jean-Herve},
  journal={Journal of Engineering Mechanics},
  volume={117},
  number={4},
  pages={907--922},
  year={1991},
  publisher={American Society of Civil Engineers}
}

@article{Schrefler1995Shear,
author = {Schrefler, Bernhard A and Majorana, Carmelo E and Sanavia, Lorenzo},
journal = {Archives of Mechanics},
mendeley-groups = {Dynamics_poromechancis,Dynamics_Unsat_Soils},
title = {{Shear band localization in saturated porous media}},
volume = {47},
year = {1995}
}

@Article{Zienkiewicz1990Static,
  author    = {Zienkiewicz, O. C. and Chan, A. H.C. and Pastor, M. and Paul, D. K. and Shiomi, T.},
  journal   = {Proceedings of the Royal Society of London. A. Mathematical and Physical Sciences},
  title     = {{Static and dynamic behaviour of soils : a rational approach to quantitative solutions. I. Fully saturated problems}},
  year      = {1990},
  month     = {jun},
  number    = {1877},
  pages     = {285--309},
  volume    = {429},
  publisher = {The Royal Society London},
}

@article{heider2014dynamic,
  title={The dynamic response of fluid-saturated porous materials with application to seismically induced soil liquefaction},
  author={Heider, Y and Avci, O and Markert, B and Ehlers, W},
  journal={Soil Dynamics and Earthquake Engineering},
  volume={63},
  pages={120--137},
  year={2014},
  publisher={Elsevier}
}

@article{Zhang2001Numerical,
author = {Zhang, H. W. and Sanavia, L. and Schrefler, B. A.},
journal = {Computers and Structures},
mendeley-groups = {Dynamics_Unsat_Soils},
month = {feb},
number = {4},
pages = {441--459},
publisher = {Elsevier Science Ltd},
title = {{Numerical analysis of dynamic strain localization in initially water saturated dense sand with a modified generalized plasticity model}},
volume = {79},
year = {2001}
}

@book{zienkiewicz1999computational,
  title={Computational geomechanics},
  author={Zienkiewicz, Olgierd C and Chan, AHC and Pastor, M and Schrefler, BA and Shiomi, T},
  volume={613},
  year={1999},
  publisher={Citeseer}
}

@article{cosserat1909theorie,
  title={Th{\'e}orie des corps d{\'e}formables},
  author={Cosserat, Eugene and Cosserat, Fran{\c{c}}ois},
  year={1909},
  publisher={A. Hermann et fils,}
}

@article{zhang2019coupling,
  title={A coupling peridynamic approach for the consolidation and dynamic analysis of saturated porous media},
  author={Zhang, Hongwu and Li, Hui and Ye, Hongfei and Zheng, Yonggang},
  journal={Computational Mechanics},
  volume={64},
  number={4},
  pages={1097--1113},
  year={2019},
  publisher={Springer}
}

@article{newmark1959method,
  title={A method of computation for structural dynamics},
  author={Newmark, Nathan M},
  journal={Journal of the engineering mechanics division},
  volume={85},
  number={3},
  pages={67--94},
  year={1959},
  publisher={American Society of Civil Engineers}
}

@article{hashim2020implicit,
  title={An implicit non-ordinary state-based peridynamics with stabilised correspondence material model for finite deformation analysis},
  author={Hashim, Nur A and Coombs, WM and Augarde, CE and Hattori, G},
  journal={Computer Methods in Applied Mechanics and Engineering},
  volume={371},
  pages={113304},
  year={2020},
  publisher={Elsevier}
}

@article{fang2021stable,
  title={A stable non-ordinary state-based peridynamic model for laminated composite materials},
  author={Fang, Guodong and Liu, Shuo and Liang, Jun and Fu, Maoqing and Wang, Bing and Meng, Songhe},
  journal={International Journal for Numerical Methods in Engineering},
  volume={122},
  number={2},
  pages={403--430},
  year={2021},
  publisher={Wiley Online Library}
}

@article{markert2010comparison,
  title={Comparison of monolithic and splitting solution schemes for dynamic porous media problems},
  author={Markert, B and Heider, Y and Ehlers, W},
  journal={International journal for numerical methods in engineering},
  volume={82},
  number={11},
  pages={1341--1383},
  year={2010},
  publisher={Wiley Online Library}
}

@article{Jabakhanji2015peridynamic,
author = {Jabakhanji, Rami and Mohtar, Rabi H.},
journal = {Advances in Water Resources},
keywords = {Derivative-free model,Flow,Non-local model,Peridynamics,Soil cracking,Unsaturated soil},
pages = {22--35},
publisher = {Elsevier Ltd},
title = {{A peridynamic model of flow in porous media}},
volume = {78},
year = {2015}
}

@article{ouchi2015fully,
author = {Ouchi, Hisanao and Katiyar, Amit and York, Jason and Foster, John T. and Sharma, Mukul M.},
journal = {Computational Mechanics},
mendeley-groups = {IJNME{\_}2019{\_}MS,Sinkholes-Aug'19,Stabilized-PD},
number = {3},
pages = {561--576},
title = {{A fully coupled porous flow and geomechanics model for fluid driven cracks: a peridynamics approach}},
volume = {55},
year = {2015}
}

@article{popescu2006dynamics,
  title={Dynamics of nonlinear porous media with applications to soil liquefaction},
  author={Popescu, Radu and Prevost, Jean H and Deodatis, George and Chakrabortty, Pradipta},
  journal={Soil dynamics and earthquake engineering},
  volume={26},
  number={6-7},
  pages={648--665},
  year={2006},
  publisher={Elsevier}
}

@article{alonso2003influence,
  title={Influence of rainfall on the deformation and stability of a slope in overconsolidated clays: a case study},
  author={Alonso, EE and Gens, Antonio and Delahaye, CH},
  journal={Hydrogeology journal},
  volume={11},
  number={1},
  pages={174--192},
  year={2003},
  publisher={Springer}
}

@article{DeBorst1991Simulation,
author = {{De Borst}, Rene},
journal = {Engineering Computations},
number = {4},
pages = {317--332},
title = {{Simulation of strain localization: A reappraisal of the cosserat continuum}},
volume = {8},
year = {1991}
}

@article{Silling2000Reformulation,
author = {Silling, S.A.},
journal = {Journal of the Mechanics and Physics of Solids},
month = {jan},
number = {1},
pages = {175--209},
publisher = {Pergamon},
title = {{Reformulation of elasticity theory for discontinuities and long-range forces}},
volume = {48},
year = {2000}

}@article{diebels1996dynamic,
  title={Dynamic analysis of a fully saturated porous medium accounting for geometrical and material non-linearities},
  author={Diebels, Stegan and Ehlers, Wolfgang},
  journal={International Journal for numerical methods in Engineering},
  volume={39},
  number={1},
  pages={81--97},
  year={1996},
  publisher={Wiley Online Library}
}

@article{schanz2000transient,
  title={Transient wave propagation in a one-dimensional poroelastic column},
  author={Schanz, Martin and Cheng, AH-D},
  journal={Acta Mechanica},
  volume={145},
  number={1-4},
  pages={1--18},
  year={2000},
  publisher={Springer}
}

@article{pastor2000fractional,
  title={A fractional step algorithm allowing equal order of interpolation for coupled analysis of saturated soil problems},
  author={Pastor, M and Li, T and Liu, X and Zienkiewicz, OC and Quecedo, M},
  journal={Mechanics of Cohesive-frictional Materials: An International Journal on Experiments, Modelling and Computation of Materials and Structures},
  volume={5},
  number={7},
  pages={511--534},
  year={2000},
  publisher={Wiley Online Library}
}

@article{needleman1988material,
  title={Material rate dependence and mesh sensitivity in localization problems},
  author={Needleman, A},
  journal={Computer methods in applied mechanics and engineering},
  volume={67},
  number={1},
  pages={69--85},
  year={1988},
  publisher={Elsevier}
}

@article{schrefler1996multiphase,
  title={A multiphase medium model for localisation and postlocalisation simulation in geomaterials},
  author={Schrefler, BA and Sanavia, L and Majorana, CE},
  journal={Mechanics of Cohesive-frictional Materials: An International Journal on Experiments, Modelling and Computation of Materials and Structures},
  volume={1},
  number={1},
  pages={95--114},
  year={1996},
  publisher={Wiley Online Library}
}

@article{de1993one,
  title={One-dimensional transient wave propagation in fluid-saturated incompressible porous media},
  author={de Boer, Reint and Ehlers, Wolfgang and Liu, Zhangfang},
  journal={Archive of Applied Mechanics},
  volume={63},
  number={1},
  pages={59--72},
  year={1993},
  publisher={Springer}
}

@article{shahbodagh2014dynamic,
  title={Dynamic analysis of strain localization in water-saturated clay using a cyclic elasto-viscoplastic model},
  author={Shahbodagh Khan, B and Mirjalili, M and Kimoto, S and Oka, F},
  journal={International Journal for Numerical and Analytical Methods in Geomechanics},
  volume={38},
  number={8},
  pages={771--793},
  year={2014},
  publisher={Wiley Online Library}
}

@article{oka2019computational,
  title={A computational model for dynamic strain localization in unsaturated elasto-viscoplastic soils},
  author={Oka, Fusao and Shahbodagh, Babak and Kimoto, Sayuri},
  journal={International Journal for Numerical and Analytical Methods in Geomechanics},
  volume={43},
  number={1},
  pages={138--165},
  year={2019},
  publisher={Wiley Online Library}
}

@inproceedings{littlewood2011nonlocal,
  title={A nonlocal approach to modeling crack nucleation in AA 7075-T651},
  author={Littlewood, David J},
  booktitle={ASME 2011 international mechanical engineering congress and exposition},
  pages={567--576},
  year={2011},
  organization={American Society of Mechanical Engineers Digital Collection}
}

@article{breitenfeld2014non,
  title={Non-ordinary state-based peridynamic analysis of stationary crack problems},
  author={Breitenfeld, MS and Geubelle, Philippe H and Weckner, O and Silling, SA},
  journal={Computer Methods in Applied Mechanics and Engineering},
  volume={272},
  pages={233--250},
  year={2014},
  publisher={Elsevier}
}

@article{extendedTupek2014,
author = {Tupek, M. R. and Radovitzky, R.},
journal = {Journal of the Mechanics and Physics of Solids},
number = {1},
pages = {82--92},
publisher = {Elsevier},
title = {{An extended constitutive correspondence formulation of peridynamics based on nonlinear bond-strain measures}},
volume = {65},
year = {2014}
}

@article{silling2017stability,
  title={Stability of peridynamic correspondence material models and their particle discretizations},
  author={Silling, Stewart A},
  journal={Computer Methods in Applied Mechanics and Engineering},
  volume={322},
  pages={42--57},
  year={2017},
  publisher={Elsevier}
}

@article{Chen2018Bond,
author = {Chen, Hailong},
journal = {Mechanics Research Communications},
pages = {34--41},
publisher = {Elsevier Ltd},
title = {{Bond-associated deformation gradients for peridynamic correspondence model}},
volume = {90},
year = {2018}
}

@article{Yaghoobi2017Higher,
author = {Yaghoobi, Amin and Chorzepa, Mi G.},
journal = {Computers and Structures},
month = {aug},
pages = {63--79},
publisher = {Elsevier Ltd},
title = {{Higher-order approximation to suppress the zero-energy mode in non-ordinary state-based peridynamics}},
volume = {188},
year = {2017}
}

@article{Gu2018Revisit,
author = {Gu, Xin and Madenci, Erdogan and Zhang, Qing},
journal = {Engineering Fracture Mechanics},
pages = {31--52},
publisher = {Elsevier Ltd},
title = {{Revisit of non-ordinary state-based peridynamics}},
volume = {190},
year = {2018}
}

@article{wang2020strain,
  title={Strain localization in non-isothermal unsaturated porous media considering material heterogeneity with stabilized mixed finite elements},
  author={Wang, Kaiqi and Song, Xiaoyu},
  journal={Computer Methods in Applied Mechanics and Engineering},
  volume={359},
  pages={112770},
  year={2020},
  publisher={Elsevier}
}

@article{Oterkus2017Fully,
author = {Oterkus, Selda and Madenci, Erdogan and Oterkus, Erkan},
journal = {Engineering Geology},
pages = {19--28},
title = {{Fully coupled poroelastic peridynamic formulation for fluid-filled fractures}},
volume = {225},
year = {2017}
}

@article{seed1967analysis,
  title={Analysis of soil liquefaction: Niigata earthquake},
  author={Seed, H Bolton and Idriss, Izzat M},
  journal={Journal of the Soil Mechanics and Foundations Division},
  volume={93},
  number={3},
  pages={83--108},
  year={1967},
  publisher={ASCE}
}

@article{Prevost1985Wave,
author = {Prevost, Jean H.},
doi = {10.1016/0261-7277(85)90038-5},
journal = {International Journal of Soil Dynamics and Earthquake Engineering},
month = {oct},
number = {4},
pages = {183--202},
publisher = {Elsevier},
title = {{Wave propagation in fluid-saturated porous media: An efficient finite element procedure}},
volume = {4},
year = {1985}
}

@article{song2017strain,
  title={Strain localization in a solid-water-air system with random heterogeneity via stabilized mixed finite elements},
  author={Song, Xiaoyu and Ye, Ming and Wang, Kaiqi},
  journal={International Journal for Numerical Methods in Engineering},
  volume={112},
  number={13},
  pages={1926--1950},
  year={2017},
  publisher={Wiley Online Library}
}

@article{eringen1964nonlinear,
  title={Nonlinear theory of simple micro-elastic solids—I},
  author={Eringen, A Cemal and Suhubi, ES},
  journal={International Journal of Engineering Science},
  volume={2},
  number={2},
  pages={189--203},
  year={1964},
  publisher={Elsevier}
}

@article{kroner1967elasticity,
  title={Elasticity theory of materials with long range cohesive forces},
  author={Kr{\"o}ner, E},
  journal={International Journal of Solids and Structures},
  volume={3},
  number={5},
  pages={731--742},
  year={1967},
  publisher={Citeseer}
}

@article{Silling2007Peridynamic,
author = {Silling, S. A. and Epton, M. and Weckner, O. and Xu, J. and Askari, E.},
journal = {Journal of Elasticity},
number = {2},
pages = {151--184},
pmid = {248806300004},
title = {{Peridynamic states and constitutive modeling}},
volume = {88},
year = {2007}
}

@article{silling2005meshfree,
author = {Silling, Stewart A and Askari, Ebrahim},
journal = {Computers {\&} structures},
number = {17-18},
pages = {1526--1535},
publisher = {Elsevier},
title = {{A meshfree method based on the peridynamic model of solid mechanics}},
volume = {83},
year = {2005}
}

@incollection{breuer1999quasi,
  title={Quasi-static and dynamic behavior of saturated porous media with incompressible constituents},
  author={Breuer, Stefan},
  booktitle={Porous Media: Theory and Experiments},
  pages={285--303},
  year={1999},
  publisher={Springer}

}

@article{ni2020hybrid,
  title={Hybrid FEM and peridynamic simulation of hydraulic fracture propagation in saturated porous media},
  author={Ni, Tao and Pesavento, Francesco and Zaccariotto, Mirco and Galvanetto, Ugo and Zhu, Qi-Zhi and Schrefler, Bernhard A},
  journal={Computer Methods in Applied Mechanics and Engineering},
  volume={366},
  pages={113101},
  year={2020},
  publisher={Elsevier}
}


